Learning Facial Liveness Representation for Domain Generalized Face Anti-spoofing

Face anti-spoofing (FAS) aims at distinguishing face spoof attacks from the authentic ones, which is typically approached by learning proper models for performing the associated classification task. In practice, one would expect such models to be generalized to FAS in different image domains. Moreover, it is not practical to assume that the type of spoof attacks would be known in advance. In this paper, we propose a deep learning model for addressing the aforementioned domain-generalized face anti-spoofing task. In particular, our proposed network is able to disentangle facial liveness representation from the irrelevant ones (i.e., facial content and image domain features). The resulting liveness representation exhibits sufficient domain invariant properties, and thus it can be applied for performing domain-generalized FAS. In our experiments, we conduct experiments on five benchmark datasets with various settings, and we verify that our model performs favorably against state-of-the-art approaches in identifying novel types of spoof attacks in unseen image domains.

==> 2.RelatedWork.tex <==
\section{Related Work}
\subsection{Face Anti-Spoofing}

The problem of FAS is typically approached by the following strategies. Utilizing handcrafted feature descriptors, previous methods including LBP~\cite{boulkenafet2015face, de2012lbp, de2013can, maatta2011face}, HoG~\cite{komulainen2013context, yang2013face}, SIFT~\cite{patel2016secure}, and SURV~\cite{boulkenafet2016face} have been applied for solving FAS using the associated features, followed by a trained binary classifier for predicting the authenticity of the input face image. With the development of deep learning approaches, various methods apply convolutional neural networks (CNN)~\cite{krizhevsky2012imagenet} to extract more discriminative features, achieving significant improvements. Feng~\cite{feng2016integration} regarded FAS as a binary classification task via a CNN architecture. Additional auxiliary supervision such as depth map, reflection map, and r-ppg signals are also considered for improving the FAS classification performances. Recently, Zhang~\cite{zhang2020face} and Liu~\cite{liu2020disentangling} extracted liveness features from the perspective of disentanglement. Although such techniques have shown promising performances, it is not clear how their extracted liveness features can be generalized across image domains/datasets, or to handle novel spoof attacks. 

\subsection{Domain Generalization}
Domain generalization aims at leveraging information learned from source domains to target domains that are unseen during training. To address FAS across image domains, Shao~\cite{shao2019multi} proposed a multi-adversarial discriminative deep domain generalization (MADDG) framework. With a dual-force triplet-mining constraint, their proposed architecture learns a generalized feature space for real and fake faces. Extended from MADDG, Jia~\cite{jia2020single} designed a single side triplet-mining algorithm, which performs FAS while grouping spoof types across domains for the purpose of domain generalization. On the other hand, Liu~\cite{liu2021dual} proposed a Dual Reweighting Domain Generalization (DRDG) framework which reweights the samples from different domains during training, aiming to separate real and fake images disregard their image domains. While the above works have shown improved generalization ability on unseen domains for FAS, it is not clear whether they can handle novel spoof attacks, and thus their usage for practical FAS tasks might still be limited. 

\subsection{Representation Disentanglement}
Representation disentanglement focuses on extracted particular feature representations, which would describe the information of interest, typically benefiting the downstream learning tasks. For FAS,~\cite{wang2020cross} proposed to jointly perform disentangled representation learning and multi-domain feature learning for cross-domain face PAD.~\cite{zhang2020face} chose to disentangle the liveness features from the feature representation of the input image, with both low-level and high-level auxiliary supervision to improve the generalization abilities. Nevertheless, these methods did not take the scenario that the target domain may not be presented during training, and the type of spoof attacks might not be novel to the existing ones. This is the reason why, as we detail in the following section, we propose to learn domain-invariant facial liveness representation for FAS. Moreover, since liveness-irrelevant information such as facial content and image domains are disentangled from the derived liveness representation, domain-generalized FAS can be achieved.


